"AI Slop is DDoSing Open Source": Understanding the Impact of AI-Generated Contributions on Open Source Sustainability

Open source software (OSS) communities are facing increasing pressure from Generative AI (GenAI) tools. We call it AI-DDoS: a denial-of-service effect in which plausible but low-quality AI-generated contributions overwhelm OSS community capacity. Using a phenomenon-based mixed-methods approach, we first analyze practitioner accounts from Reddit, OSS mentor mailing lists, and blogs to identify six recurring themes and derive hypotheses. We then evaluate these hypotheses using Bayesian Structural Time Series analysis across 294 repositories with over 2 million pull requests and issues. Our results show that while PR volume increased in 2025, merge rates declined, with one-time contributors experiencing an 18.18% drop in PR merge rates relative to the counterfactual. Finally, we identify 11 remediation strategies through practitioners' interviews and validate them with a survey of 229 OSS practitioners, grouping them into preservative, adaptive, and transformative orientations. Our findings show that AI-DDoS is not only a contribution-volume problem but a sustainability trap: communities often default to low-effort defensive strategies that protect short-term review capacity while making openness difficult to sustain.

==> sections/7_Conclusion.tex <==
\section{Conclusion}

OSS is experiencing structural pressure from AI-assisted contributions. We characterize this pressure as AI-DDoS: a denial-of-service effect in which floods of low-quality AI-assisted contributions exhaust community capacity. We synthesized and survey-validated 11 remediation strategies spanning preservative, adaptive, and transformative categories. However, our results also show that current community responses remain concentrated around low-cost, low-effort preservative strategies, leaving deeper adaptive and transformative responses underdeveloped. Our future research agenda is to help OSS communities survive and transform under the pressure of AI-assisted contributions by designing infrastructures that sustain openness in the AI era.
